Analysis of ion chain sympathetic cooling and gate dynamics

Sympathetic cooling is a technique often employed to mitigate motional heating in trapped-ion quantum computers. However, choosing system parameters such as number of coolants and cooling duty cycle for optimal gate performance requires evaluating trade-offs between motional errors and other slower errors such as qubit dephasing. The optimal parameters depend on cooling power, heating rate, and ion spacing in a particular system. In this study, we aim to analyze best practices for sympathetic cooling of long chains of trapped ions using analytical and computational methods. We use a case study to show that optimal cooling performance is achieved when coolants are placed at the center of the chain and provide a perturbative upper-bound on the cooling limit of a mode given a particular set of cooling parameters. In addition, using computational tools, we analyze the trade-off between the number of coolant ions in a chain and the center-of-mass mode heating rate. We also show that cooling as often as possible when running a circuit is optimal when the qubit coherence time is otherwise long. These results provide a roadmap for how to choose sympathetic cooling parameters to maximize circuit performance in trapped ion quantum computers using long chains of ions.

==> coverletter.tex <==

Dear Editor,

We write to you today regarding the submission of our research article, "Analysis of ion chain sympathetic cooling and gate dynamics". In this article, we present an analysis of laser cooling schemes for trapped-ion quantum computing, examining the impact of system parameters such as coolant placement in a long chain and cooling time on average entangling gate fidelity. We find that in all cases examined, placing coolant ions at the center of the chain while cooling as often as possible is always optimal for the examined sets of system parameters. 

This work is the first look at specific parameters and trade-offs when implementing cooling schemes for increased performance of long-chain trapped-ion quantum computers, a leading platform in quantum information processing. This article explicitly ties chain cooling dynamics and relevant system parameters, through theory and simulation, to widely-used figures of merit for trapped-ion quantum computing, providing a roadmap on how to improve trapped-ion quantum computer performance. Our quantitative results can likewise be generalized into qualitative heuristics and best-practices. In addition, the computational methods presented in this paper can be used to calibrate relevant parameters for practical implementation.

We believe our work would appeal to the readership of Physical Review Applied due to the immediate application to improving trapped ion quantum computer performance, a leading quantum information processing platform.
Our work jointly uses analytical and computational approaches to shed new light on trapped-ion heating and cooling while tying these results directly to relevant figures of merit for quantum computing, such as entangling gate fidelity. By examining these dynamics over a range of possible system parameters, we not only examine ways to improve system performance through calibration, but also how system performance changes with hardware improvements achievable in the near term. 

Thank you for your time and consideration.

Sincerely,
Aditya Paul and Crystal Noel

Suggested Reviewers:
Rajibul Islam (University of Waterloo)
Philipp Schindler (Univeristy of Innsbruck, Austria)
Luming Duan (Tsinghua University, China)
Allison Carter (NIST - Boulder)



100 words: Our work is a good fit for Physical Review Applied as it probes the physical dynamics of trapped ions and how to engineer system parameters for high-performance trapped-ion quantum computing. By using our physical model to examine cooling dynamics and gate performance over a variety of real system parameters, we analyze the effect of near-term hardware improvements on trapped-ion cooling performance, linking our theoretical findings to experimental results and establishing a clear tie to the future of trapped-ion quantum computing.

Summary:
In this paper, we present an analysis of laser cooling schemes for trapped-ion quantum computing, examining the impact of system parameters such as coolant placement in a long chain and cooling time on average entangling gate fidelity. We find that in all cases examined, placing coolant ions at the center of a chain while cooling as often as possible is always optimal for all examined sets of system parameters. Our quantitative results can likewise be generalized into qualitative heuristics and best-practices.





Notes:


from the journal website:
- bridge the gap between engineering and physics, and between current and future technologies. 
    - Examines system dynamics as a function of design parameters specifically as it pertains to relevant figures of merit for trapped-ion quantum computing (done)
- PRApplied publishes research with strong and clear ties to applications, and that offers fresh insight into physical phenomena. 
    - clear tie to future of trapped ion quantum computing
    - Using computational dynamics models in order to analyze the impact of specific hardware changes on a quantum system (done)
    - chain cooling dynamics with real system parameters (done)
    - immediate implications for trapped ion quantum computing
- topic area = Quantum information processing, both algorithms and hardware

criteria:
Present fresh insight into applications-based physical phenomena.
    We explore trapped-ion quantum computing from a theoretically-motivated perspective, while using computational methods to bridge the gap between the theory and experimental results. (done)
Make a significant contribution in a specific research area and generate interest for PRApplied's readers.
    first look at specific parameters and trade-offs when actually implementing schemes previously proposed towareds highest possibly performance of trapped ion quantum computers, a leading platform in QIP (done)
Represent an authoritative and substantive addition to the body of literature.
    Explicitly ties chain cooling dynamics, through theory and simulation, to widely-used figures of merit for trapped-ion quantum computing, providing a roadmap on how to improve cooling schemes and trapped-ion quantum computer performance. (done)
Explore the subject matter comprehensively and thoroughly.
    We examine cooling dynamics and quantum computer performance through both analytical and computational approaches over a variety of relevant system parameters. (done)
    We present quantitative results that can likewise be generalized into qualitative heuristics and best-practices for implementing cooling schemes on trapped-ion quantum computers (done)
